Survey of Low-Resource Machine Translation

We present a survey covering the state of the art in low-resource machine translation research. There are currently around 7000 languages spoken in the world and almost all language pairs lack significant resources for training machine translation models. There has been increasing interest in research addressing the challenge of producing useful translation models when very little translated training data is available. We present a summary of this topical research field and provide a description of the techniques evaluated by researchers in several recent shared tasks in low-resource MT.

==> figs/hierarchy.tex <==


\tikzset{
  basic/.style  = {draw, text width=2cm, drop shadow, font=\sffamily, rectangle},
  root/.style   = {basic, rounded corners=2pt, thin, align=center, fill=white},
  level-2/.style = {basic, rounded corners=6pt, thin,align=center, fill=white, text width=2.3cm},
  level-3/.style = {basic, thin, align=center, fill=white, text width=1.8cm},
  level-4/.style = {basic, thin, align=center, fill=white, text width=1.8cm, text width=1.5cm}
}

\begin{figure}
    \centering
\begin{tikzpicture}[
  level 1/.style={sibling distance=12em, level distance=5em, text width=6cm},
%   {edge from parent fork down},
  edge from parent/.style={->,solid,black,thick,sloped,draw}, 
  edge from parent path={(\tikzparentnode.south) -- (\tikzchildnode.north)},
  >=latex, node distance=1.2cm, edge from parent fork down
  ]

% root of the the initial tree, level 1
\node[root] {\textbf{Low-resource NMT}}
% The first level, as children of the initial tree
  child {node[level-2, xshift=-1.5cm] (c1) {\textbf{Data \\collection}}}
  child {node[level-2, text width=4cm] (c2) {\textbf{Exploiting available data/resources}}}
  child {node[level-2, xshift=1.5cm] (c3) {\textbf{Model \\choices}}};
  %child {node[level-2] (c4) {\textbf{Category 4}}};

% The second level, relatively positioned nodes
\begin{scope}[every node/.style={level-3}]
\node [below of = c1, xshift=10pt] (c11) {item 1-1};
\node [below of = c11] (c12) {item 1-2};
\node [below of = c12] (c13) {item 1-3};

\node [below of = c2, yshift=-10pt] (c22) {Multilingual data};
\node [left=5mm of c22] (c21) {Monolingual data};
\node [right=5mm of c22] (c23) {Linguistic resources};

\node [below of = c3, xshift=10pt] (c31) {item 3-1};
\node [below of = c31] (c32) {item 3-2};
\node [below of = c32] (c33) {item 3-3};
\node [below of = c33] (c34) {item 3-4};
\node [below of = c34] (c35) {item 3-5};

%\node [below of = c4, xshift=10pt] (c41) {item 4-1};
%\node [below of = c41] (c42) {item 4-2};
\end{scope}

% The third level, relatively positioned nodes
\begin{scope}[every node/.style={level-4}]

% Uses of monolingual data
\node [below of = c21, xshift=10pt] (c211) {\scriptsize External LMs};
\node [below of = c211] (c212) {\scriptsize Parallel data synthesis};
\node [below of = c212] (c213) {\scriptsize Parallel data modification};

% Uses of external resources
\node [below of = c23, xshift=10pt] (c231) {\scriptsize Linguistic tools};
\node [below of = c231] (c232) {\scriptsize Bilingual lexicons};

% Uses of multilingual data (TO DO)

% Uses of linguistic resources (TO DO)

\end{scope}

% lines from each level 1 node to every one of its "children"
\foreach \value in {1,2,3}
  \draw[->] (c1.195) |- (c1\value.west);

\foreach \value in {1,...,3}
  \draw[->] (c2) |- (c2\value.north);

\foreach \value in {1,...,5}
  \draw[->] (c3.195) |- (c3\value.west);
  
\foreach \value in {1,...,3}
  \draw[->] (c21.195) |- (c21\value.west);
  
  \foreach \value in {1,...,2}
  \draw[->] (c23.195) |- (c23\value.west);
  
\end{tikzpicture}
    \caption{This is a simple Taxonomy}
    \label{fig:my_label}
\end{figure}

==> nocite.tex <==
\nocite{ataman2019latent}
\nocite{sennrich2019revisiting}
\nocite{koehn2017six}
\nocite{gibadullin2019survey}
\nocite{bojar-tamchyna-2011-improving}
\nocite{bertoldi-federico-2009-domain}
\nocite{currey2017copied}
\nocite{lample-etal-2018-phrase}
\nocite{lample2018unsupervised}
\nocite{artetxe2018unsupervised}
\nocite{lample2018phrase}
\nocite{artetxe-etal-2018-robust}
\nocite{fadaee2017data}
\nocite{baziotis2020language}
\nocite{stahlberg-etal-2018-simple}
\nocite{cheng2016semi}
\nocite{tu2016neural}
\nocite{zhang-zong-2016-exploiting}
\nocite{domhan-hieber-2017-using}
\nocite{peters-etal-2018-deep}
\nocite{zhu2020incorporating}
\nocite{imamura-sumita-2019-recycling}
\nocite{clinchant-etal-2019-use}
\nocite{yang2020making}
\nocite{song2019mass}
\nocite{edunov-etal-2019-pre}
\nocite{niehues-cho-2017-exploiting}
\nocite{garciamartinez:hal-01433161}
\nocite{huck-etal-2019-better}
\nocite{aharoni-goldberg-2017-towards}
\nocite{tamchyna-etal-2017-modeling}
\nocite{eriguchi-etal-2016-tree}
\nocite{nadejde-etal-2017-predicting}
\nocite{dong-etal-2015-multi}
\nocite{luong2016multitask}
\nocite{alexandrescu-kirchhoff-2006-factored}
\nocite{burlot-etal-2017-word}
\nocite{koehn-hoang-2007-factored}
\nocite{sennrich-haddow-2016-linguistic}
\nocite{arthur-etal-2016-incorporating}
\nocite{kaiser-learning_2017}
\nocite{duan-etal-2020-bilingual}
\nocite{feng-etal-2017-memory}
\nocite{Nag2019-es}
\nocite{dinu-etal-2019-training}
\nocite{post-vilar-2018-fast}
\nocite{ijcai2020-0496}
\nocite{nguyen2017transfer}
\nocite{kocmi2018trivial}
\nocite{zhang2020improving}
\nocite{gu2018meta}
\nocite{zhou2019handling}
\nocite{zoph2016transfer}
\nocite{gu2018universal}
\nocite{guzman2019flores}
\nocite{devlin2018bert}
\nocite{artetxe2017learning}
\nocite{nguyen-chiang-2018-improving}
\nocite{firat-etal-2016-multi}
\nocite{johnson2017google}
\nocite{zaremoodi2018adaptive}
\nocite{aharoni2019massively}
\nocite{hoang2018iterative}
\nocite{sanchez-understanding-2020}
\nocite{sennrich2016improving}
\nocite{ramesh2018neural}
\nocite{neubig2018rapid}
\nocite{gulcehre2017integrating}
\nocite{kim2019effective}
\nocite{zaremoodi-haffari-2019-adaptively}
\nocite{mueller2020analysis}
\nocite{siddhant-etal-2020-leveraging}
\nocite{Dabre2020-bb}
\nocite{goyal-etal-2020-efficient}
\nocite{nekoto2020participatory}
\nocite{Cheng2020-tz}
\nocite{Eikema2020-dl}
\nocite{tambouratzis2017machine}
\nocite{adams-EtAl:2017:EACLlong}
\nocite{chen-EtAl:2017:Long5}
\nocite{ws-2019-technologies}
\nocite{tracey-etal-2019-corpus}
\nocite{philip2020revisiting}
\nocite{Tiedemann2020-sg}
\nocite{liu2020multilingual}
\nocite{Tan2019-iq}
\nocite{Zhong2020-ou}
\nocite{Pavlick-EtAl-2014:TACL}
\nocite{barrault-EtAl:2019:WMT}
\nocite{li-etal-2019-niutrans}
\nocite{bawden-etal-2019-university}
\nocite{zhu2019incorporating}
\nocite{radford2018improving}
\nocite{radfordlanguage}
\nocite{lample2019cross}
\nocite{Lewis2019-ry}
\nocite{khayrallah2020simulated}
\nocite{2019arXiv190705791S}
\nocite{schwenk2019ccmatrix}
\nocite{banon-etal-2020-paracrawl}
\nocite{haddow2020pmindia}
\nocite{siripragada-etal-2020-multilingual}
\nocite{zhang-etal-2020-chren}
\nocite{hasan-etal-2020-low}
\nocite{vaswani2017attention}
\nocite{stahlberg2019nmt}
\nocite{wang2020exposure}
\nocite{NEURIPS2019_f4d0e2e7}
\nocite{Eikema2019}
\nocite{effective2019pelsmaeker}
\nocite{setiawan-etal-2020-variational}
\nocite{muller2019domain}
\nocite{wiseman-rush-2016-sequence}
\nocite{shen-etal-2016-minimum}
\nocite{ranzato2016sequence}
\nocite{zhang-etal-2019-bridging}
\nocite{naskar2020energybased}
\nocite{tu2020engine}
\nocite{liu2018proceedings}
\nocite{fraserfindings}
\nocite{wang-etal-2020-multi-task}
\nocite{marchisio-duh-koehn:2020:WMT}
\nocite{kim-etal-2020-unsupervised}
\nocite{edman-etal-2020-low}
\nocite{hedderich-etal-2020-transfer}
\nocite{chronopoulou-etal-2020-reusing}
\nocite{araabi-monz-2020-optimizing}
\nocite{sanchez-cartagena-etal-2020-understanding}
\nocite{feldman-coto-solano-2020-neural}
\nocite{xu-etal-2020-dynamic}
\nocite{chakrabarty-etal-2020-improving}
\nocite{ngoc-le-sadat-2020-revitalization}
\nocite{li-etal-2020-emergent}

